Coz: Finding Code that Counts with Causal Profiling

Improving performance is a central concern for software developers. To locate optimization opportunities, developers rely on software profilers. However, these profilers only report where programs spent their time: optimizing that code may have no impact on performance. Past profilers thus both waste developer time and make it difficult for them to uncover significant optimization opportunities. This paper introduces causal profiling. Unlike past profiling approaches, causal profiling indicates exactly where programmers should focus their optimization efforts, and quantifies their potential impact. Causal profiling works by running performance experiments during program execution. Each experiment calculates the impact of any potential optimization by virtually speeding up code: inserting pauses that slow down all other code running concurrently. The key insight is that this slowdown has the same relative effect as running that line faster, thus "virtually" speeding it up. We present Coz, a causal profiler, which we evaluate on a range of highly-tuned applications: Memcached, SQLite, and the PARSEC benchmark suite. Coz identifies previously unknown optimization opportunities that are both significant and targeted. Guided by Coz, we improve the performance of Memcached by 9%, SQLite by 25%, and accelerate six PARSEC applications by as much as 68%; in most cases, these optimizations involve modifying under 10 lines of code.

==> Makefile <==
MAIN 			:= main

PDFLATEX  := pdflatex -halt-on-error -interaction nonstopmode
BIBTEX		:= bibtex

TEX      := $(wildcard *.tex)
BIB      := $(wildcard *.bib)
RSCRIPTS := $(wildcard r/*.r)
PLOTS    := $(patsubst r/%.r,plots/%.pdf,$(RSCRIPTS))
FIGS     := $(wildcard figures/*.pdf)
OUTPUT   := $(addsuffix .pdf,$(MAIN))
AUX      := $(addsuffix .aux,$(MAIN))

FIND_BIB_CMD := grep -l \\\\bibliography{ $(TEX)
TEX_WITH_BIB := $(shell $(FIND_BIB_CMD) )
BBL 	       := $(TEX_WITH_BIB:.tex=.bbl)

SIDE_EFFECTS := $(OUTPUT) $(AUX) $(BBL) \
							 	$(addsuffix .out,$(MAIN)) \
							 	$(addsuffix .blg,$(MAIN)) \
							 	$(addsuffix .log,$(MAIN))

all: $(AUX) $(BBL) $(OUTPUT)

clean:
	@rm -f $(SIDE_EFFECTS)

data/overhead.csv: data/overhead_unprocessed.csv data/overhead.py
	@cd data; ./overhead.py

plots/%.pdf: r/%.r data/%.csv
	@cd plots; r --no-save < ../$<

plots/hashes.pdf: r/hashes.r data/dedup_final_hashes.csv data/dedup_initial_hashes.csv
	@cd plots; r --no-save < ../r/hashes.r

$(AUX): $(TEX)
	@echo "Running pdflatex"
	@$(PDFLATEX) $(@:.aux=.tex)

$(BBL): $(TEX) $(BIB)
	@echo "Running bibtex"
	@$(BIBTEX) $(@:.bbl=.aux)

$(OUTPUT): $(TEX) $(BBL) $(PLOTS) $(FIGS)
	@echo "Running pdflatex"
	@$(PDFLATEX) $(@:.pdf=.tex) > /dev/null
	@$(PDFLATEX) $(@:.pdf=.tex) > /dev/null


==> future_work.tex <==
\section{Future Work}
\label{sec:future_work}

% Profile JIT-generated code using the GDB API
%% Place a trap in the `__jit_debug_register_code` function
%% Locate any newly created entries, process DWARF information
%% That's it! To be usable, more expressive profiler scoping will be required.

% Profile Kernel
%% Need to process Kernel debug symbol information (different format)
%% No line information, but all existing mechanisms will support both virtual speedups *and* progress points in the kernel

% Cross-process support
%% Global delay counter must be shared across processes in the group
%% Signals from other processes in the group should be handled the same way as signals from other threads.

% Profiling within a single line
%% Sometimes one line can perform a number of operations (like a for loop)
%% Causal will only measure the effect of speeding up all of them
%% DWARF format supports column information. LLVM/Clang will generate it with a special flag. This would support profiling individual statements within a single line (for loop, macro instantiation)

==> punted.tex <==
%In effect, causal profiling uses
%\emph{the program as its own performance model} to predict the impact
%of optimizations. Causal profiling can profile both throughput and
%latency via programmer-supplied progress points like transaction
%boundaries.




%Developers cannot manually optimize all of a program's code, so they rely on software profilers to find important code.
%For each code fragment, developers need to know \emph{``How much will optimizing this code improve performance?''}
%This is a question of causality, which conventional profilers cannot answer.
%Conventional profilers measure how much each fragment of code contributes to execution time.
%This is sufficient for serial programs, but not all executed code contributes to the end-to-end runtime of a parallel program.
%Recent techniques have relied on performance models to address this shortcoming, but these models can not capture the full complexity of performance on modern hardware.

%Causal profiling identifies important code by running \textit{performance experiments}.
%Each experiment uses \textit{virtual speedups} to create the effect of an optimization, and directly measures the effect of this optimization on end-to-end performance.
%There is no need to predict the effect of a performance change because a causal profiler measures it directly.


% Benchmark info
\begin{table}
  \centering
  \small
  \begin{tabular}{lll}
    \multicolumn{3}{c}{\textbf{Benchmark Details}} \\
    Benchmark     & Input Size   \\
    \hline
    blackscholes  & native       \\
    bodytrack     & native       \\
    canneal       & native       \\
    dedup         & native       \\
    facesim       & native       \\
    ferret        & native       \\
    fluidanimate  & native       \\
    freqmine      & native       \\
    raytrace      & native       \\
    streamcluster & test         \\
    swaptions     & native       \\
    vips          & native       \\
    x264          & native       \\
  \end{tabular}
\end{table}

\punt{
\subsection{OLD OVERVIEW TEXT STARTS HERE}

% Quick reminder of causal profiling, performance experiments, virtual speedups, and progress points
The purpose of a causal profiler is to identify code where optimizations will have the largest impact. To measure the impact of optimizing a single line of code, a causal profiler conducts a performance experiment. Using a technique we call virtual speedup, the profiler intentionally distorts the program's execution so it will behave as if the selected line was optimized. Meanwhile, the profiler measures the rate of visits to progress points, developer-specified points in the code where some useful work is completed. Any change in the program's rate must be the result of the virtual speedup. The results of many such experiments form a causal profile. This section gives an overview of each stage of our technique, from performance experiments to profile interpretation.

\subsection{Profile Collection}
% Select a line to speed up
To begin a performance experiment, a causal profiler randomly selects a line of code to (virtually) speed up. Rather than selecting lines uniformly at random, the profiler selects a line from the distribution of execution time. This ensures that the causal profiler is evaluating the effect of optimizing code that is actually executed. The search is biased toward frequently-executed lines. While frequently-executed code is not necessarily important for a program's performance, speeding up code that never runs is unlikely to have any effect.
% If all we did was speed up the code that never runs, it would certainly have no effect. But, it's hard to change the code without changing its size, thus changing layout.
% I'm half-inclined to claim that speeding up code that never executes cannot possible have an effect just to see if someone will quote Stabilizer back to us...

% Select a speedup amount
Once a line has been selected for speedup, the causal profiler must decide how much speedup to evaluate. A causal profiler measures all speedups as a percent-reduction in execution time:

  \[ \text{speedup} = \frac{t_{\text{original}} - t_{\text{optimized}}}{t_{\text{original}}} \]

The amount of virtual speedup applied to the selected line is chosen randomly between 0\% (no change) and 100\% (the line is completely eliminated).

% Begin the experiment
Finally, the causal profiler logs the state of all progress points and starts the performance experiment. The selected virtual speedup is applied for the duration of the experiment, after which the progress point state is logged again. The performance effect of each virtual speedup is only determined in offline profile analysis. The profiler immediately selects a new line and speedup to conduct another performance experiment.





%%% Unrevised below %%%



% Basic overview of sampling-based virtual speedups
\paragraph{Virtual speedups} create the effect of optimizing the selected line without actually speeding the line up. Instead, each time the selected line is executed in one thread, all other threads must pause. Threads that execute the selected line will run faster relative to threads that do not. The length of each pause determines the size of the virtual speedup: if all other threads pause for half the time it takes to execute the selected line, the line will appear to run 50\% faster. Effective execution time, the time that would have elapsed if the selected line really was optimized, is computed by subtracting the total amount of delay from the elapsed wall time. Figure~\ref{fig:virtual_speedup} shows this procedure graphically.

% The approach outlined above is untenable
Pausing threads every time a line is executed is problematic in practice. First, the overhead of tracking every visit to the selected line could be quite large. The largest possible pause, to create the effect of completely optimizing away the selected line, is still quite small: just the time it takes to run the selected line once. Inserting such a small delay precisely would be difficult, and we have no way of actually measuring the time it takes to run the selected line in the first place.

% Sampling can have the same effect as above without the drawbacks
Instead of using instrumentation, a causal profiler creates the speedup effect using sampling. Each thread samples its program counter at a fixed sampling period $P$. Every time a sample falls in the currently selected line, all other threads must pause for some delay size $d$. The selected line appears to run $\frac{d}{P}$ percent faster than the un-optimized version. Section~\ref{sec:analysis} shows that the sampling approach is equivalent to the impractical approach described above.

% Progress points enable faster profile collection, and support non-terminating programs
\paragraph{Progress points} are source locations, specified by the end-user, executed repeatedly by the profiled program. A causal profiler measures the time between visits to progress points to track performance mid-execution. This allows the profiler to conduct many performance experiments in a single execution, with the added benefit of supporting programs that do not terminate, or where end-to-end runtime is not meaningful.

% Use Little's Law to measure latency
Progress points also make it possible to measure the effect of an optimization on latency rather than throughput. To measure latency, the developer simply adds progress points at the beginning and end of some operation. There is no need to attach timestamps or identifiers to individual requests. Instead, we take advantage of Little's Law: $L = \lambda W$, where $L$ is the number of waiting requests, $\lambda$ is the arrival rate, and $W$ is the latency~\cite{little2011or}. The beginning progress point allows us to measure $\lambda$, and the difference in execution counts between the beginning and end points gives us $L$, the number of outstanding requests.

% Fluctuations in performance are not a threat
A program's progress rate may fluctuate during a program's execution. Repeating an experiment many times during an execution allows us to control for these fluctuations. If the average performance with a virtual speedup in place is different from baseline performance, the speedup must be responsible. Causal profiles from multiple runs can be combined, further smoothing out any noise from program phases.

\subsection{Profile Analysis}

\begin{figure}
  \centering
  \caption{
    \label{fig:speedup_curve}
    A typical speedup curve
  }
\end{figure}


% Description of speedup curves, and interpretation
Once a causal profile has been collected, developers must be able to interpret them accurately. The entire profile consists of measured program speedups for varying line speedup amounts across many lines in the program. For each line, we plot the line speedup vs. program speedup on a \emph{speedup curve}. One typical speedup curve is shown in Figure~\ref{fig:speedup_curve}. These curves show two important properties for each line of code. First, the slope of the speedup curve shows the \emph{payback rate} for optimizing this line: the steeper the line, the more effect a small optimization will have. Second, the maximum value on the speedup curve shows the \emph{maximum impact}: the largest possible performance improvement from optimizing this line of code. Ideally, developers would find lines with high values for both payback rate and maximum impact.

% Ranking lines using regressions
We use a simple linear regression to get an initial measure of a line's optimization potential. Lines are ranked by the slope of this linear regression. Lines with both large payback rate and maximum impact will have a steeper regression line. Developers may also wish to bias their search toward payback rate or maximum impact. Weighting points with low line speedup values (toward the left of the plot) will bias the regression toward payback rate, while weighting points with large line speedups will better capture maximum impact.

% Code heat map?

% Test new regression approaches:
%% Weight low-speedup points in regression to measure the bang-for-buck (slope of regression)
%% Weight high-speedup points in regression to measure the maximum impact (x=1.0 intercept)

}
\punt{
Past work has focused primarily on improving profiler accuracy by
reducing \emph{probe effect}, the distortion of a program's
execution due to profiler overhead.  Lightweight instrumentation can
reduce this effect, resulting in more accurate
profiles~\cite{DBLP:conf/sigplan/GrahamKM82}. Profilers that use
sampling exclusively nearly eliminate probe effect, although care must be
taken to ensure that sampling is truly random and
unbiased~\cite{DBLP:conf/pldi/MytkowiczDHS10}.
}
\punt{
% from abstract
Developers use profilers to identify code that should be optimized. For each piece of code, developers would like to know \emph{``How much will optimizing this code improve performance?''} This is a question of causality, which conventional profilers cannot answer. A conventional profiler measures the time spent running each function. For serial programs, a function's runtime is sufficient to infer its performance impact; however, concurrent and asynchronous programs are not so simple. Threads in a parallel program can interfere, and not all code contributes to a program's execution time.

We introduce \emph{Causal Profiling}, a novel profiling technique that relies on a series of controlled experimentation rather than passive observation. For each experiment, the profiler makes a small change to the performance of a single line of code. Any observed effect on whole-program performance must be caused by this change. After running many such experiments, a causal profiler can direct a developer to the lines of code which, if optimized, will have the greatest impact on performance.

% Discuss Cozzle, validation, experimental summary, etc.
}
\punt{
% This is because
%conventional profilers do not properly consider concurrent paths
%through a program.

% Concurrency creates multiple paths through the program.
% Actually, instructions are parallel and even serial code has a critical path...
The execution of a completely serial program follows a single path through the program's control flow graph. The length of this path is the execution time of the program. A concurrent program consists of many paths: events within each thread occur in control-flow order, but cross-thread dependencies create edges between threads forming the program activity graph~\cite{DBLP:journals/tse/YangM89}. It is the length of the longest path through this graph, the \emph{critical path}, that determines execution time. 

% Not all paths matter, but conventional profilers measure all of them.
In our simple example, every call to \cfunction{poll} that returns \cfunction{false} is off the critical path. Only speeding up the read operation will improve the program's performance. In general, a concurrent program can only be sped up by shortening its critical path. When a conventional profiler observes a concurrent program, it records time spent on all paths, not just the program's critical path. As a result, conventional profilers can lead developers to waste time tuning code where little or no performance impact is possible.

%%%%%%%%%%% How is it solved today? %%%%%%%%%%%

% Newer but infrequently used approaches specifically target concurrency: lock/contention profilers and "blame" profilers
Some profiling approaches specifically target concurrent software. Contention profilers measure the time threads spend blocked waiting for access to shared resources such as locks~\cite{goldin2010thread}. Another approach is to assign ``blame'' to code that is executing while a thread is blocked on some shared resource~\cite{DBLP:conf/sigmetrics/AndersonL90}. While both these approaches can identify possible sources of contention in concurrent programs, there is no guarantee that this contention occurs on the critical path.
% Embed a correlation != causation reference here

% Critical path profiling is not sufficient---the critical path can change. Identifying the critical path is prohibitively expensive
Yet another approach is to trace program execution to record the program activity graph~\cite{DBLP:journals/tse/YangM89}. A tracing profiler must record every interaction between threads to correctly identify the critical path. Critically, these profilers fail to consider the implications of hardware/software interaction in a concurrent program. Contention on cache lines or the memory bus can lead to significant performance problems, but tracing these operations would be prohibitively expensive~\cite{DBLP:conf/oopsla/LiuB11}.

% PAG captures order, not dependence. Any timing change could reorder the graph.
Even a complete program activity graph is not sufficient to identify code where optimizations will have a large impact. The order of operations in the PAG does not imply dependence---the ordering could be timing-dependent. Optimizing code, whether on or off the critical path, can change the order of any timing-dependent events, possibly leading to a new critical path. As a result, the program activity graph lacks predictive power.
}


\punt{

Conventional profilers typically rank a program's functions by their total execution time. Developers use this ranking as a proxy for importance, assuming that optimizing the longest-running functions will have the greatest performance impact. This assumption holds for serial programs, where execution time and impact are correlated. In concurrent programs, however, runtime and impact no longer have this predictable relationship.

Optimizing a function will only reduce a program's runtime if it is executed on the program's critical path. Conventional profilers measure all execution time, regardless of whether it is on the critical path. A function may never appear on the critical path, but if it has a large total runtime a conventional profiler will include it near the top of its ranking. Further complicating matters, the critical path may change after even small optimizations. As a result, conventional profilers may lead developers to waste time optimizing code that where little or no impact on end-to-end performance is even possible.

To measure the effect of optimizing a line of code, a causal profiler must speed up the line's execution. Ideally we could automatically improve the performance of a selected line. Unfortunately, we have to assume that any automatic means of improving performance has already been applied. Instead, a causal profiler uses \emph{virtual speedups} to 

 the line by inserting delays in other threads whenever the line is executed. Varying the size of the delay allows the profiler to measure the impact of different optimization sizes.

Progress points have other benefits, beyond making causal profiling tractable. In a large software system, placing progress points allows developers to find optimizations that will target a specific component. A causal profiler can support multiple progress points simultaneously, so developers can consider the impact of an optimization across multiple components in a large system.

Progress points also make it possible to find optimizations that will reduce latency of some operation. A developer must mark the begin and end points of the operation. There is no need to attach timestamps to individual requests. Instead, the profiler measures request arrival rate and the number of outstanding requests (the number started minus the number completed), and can compute average latency using Little's Law~\cite{little2011or}.

}

% Old accuracy experiment discussion
\subsection{Accuracy}
\label{sec:accuracy}

% We want to know if the speedups predicted by Coz correspond to reality

A causal profiler predicts the effect of optimizing a line of code.
For this profile to be useful, the predicted effect must be
accurate. Ideally, we would use \coz{} to identify a source line,
optimize the line, then compare \coz{}'s prediction to the actual
effect. Unfortunately, this labor-intensive approach would not scale
to the number of measurements required to perform a thorough
evaluation. Instead, we run \coz{} on a program after slowing down one
of its lines. We can then remove the slowdown to ``optimize'' the
line, and compare the resulting effect on performance to \coz{}'s
prediction.

\begin{figure}[!t]
  \begin{lstlisting}[language=C++,
                   directivestyle={\color{black}}
                   emph={int,char,double,float,unsigned,size_t,void,for,thread,join,true,__asm__,volatile},
                   emphstyle={\color{blue}}
                  ]
  /* Delay macro for accuracy evaluation */
  if (true) {                    \
    for (volatile int coz_i = 0; \
         coz_i < 5;              \
         coz_i++)                \
      ;                          \
     _causal_trip_count++;       \
  }
  \end{lstlisting}
\caption{
\small
An example delay macro used to verify the accuracy of \coz{}'s predictions ($\S$\ref{sec:accuracy}). We place these in the benchmarks and compare the effect of removing the delay with \coz{}'s predictions. The actual macro is a single line; we expand it here for clarity.
  \label{fig:delay-macro}
}
\end{figure}

We identify all lines in the PARSEC benchmarks that account for at
least 1\% of the benchmark's total runtime, 182 lines in total. We add
a C preprocessor macro to each of these lines, which lets us insert
delays in each line independently. When a delay is enabled, the line
maintains a trip count and executes a short
loop. Figure~\ref{fig:delay-macro} shows an example. We measure the
percent execution time with each delay in place, which lets us
determine how much we can ``optimize'' the line by removing the delay.



==> related_notes.tex <==
\subsection*{Serial Profilers}

\paragraph{Exploiting Hardware Performance Counters with Flow and Context Sensitive Profiling~\cite{DBLP:conf/pldi/AmmonsBL97}}
Extend work on efficient path profiling to flow-sensitive profiling. Use hardware performance counters, which they associate with specific paths through a procedure. Flow-sensitive information reduces ambiguity: "flow insensitive measurement might find two statements that have high cache miss rates, whereas a flow sensitive measurement could show that the misses occur when the statements execute along a common path." Also presents calling context profiling, beyond simple call-graph edge profiling.

\paragraph{Efficient Path Profiling~\cite{DBLP:conf/micro/BallL96}}
Assigns each path a unique ID. Inserts instrumentation to update a register at some (not all) block edges. At the end of the path, register holds the path ID. Significantly more precise performance information is possible with path profiles versus procedure-level profiling data.

\paragraph{gprof: a Call Graph Execution Profiler~\cite{DBLP:conf/sigplan/GrahamKM82}}
Records invocation counts for caller-callee pairs. Uses sampling to attribute runtime to each node in the call graph. Non-zero overhead (about 30\%).

\paragraph{Instant profiling: Instrumentation sampling for profiling datacenter applications~\cite{DBLP:conf/cgo/ChoMHBM13}}
Interleaves instrumented and normal execution to reduce edge profiling overhead. Supports multithreaded programs, but there's no special multithreaded-friendly profiling.

% TO ADD
\paragraph{Valgrind: a framework for heavyweight dynamic binary instrumentation~\cite{DBLP:conf/pldi/NethercoteS07}}
Dynamic binary instrumentation framework. Provides cache (Cachegrind) and heap (Massif) profiling tools, but threads are run context-switched with only one thread active at a time.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{Time Attribution}

\paragraph{Performance analysis of idle programs~\cite{DBLP:conf/oopsla/AltmanAFM10}}
Motivated by enterprise Java workloads: instrumentation and runtime modifications are not acceptable. Use periodic javacore dumps and expert rules to infer an abstract performance model. Argues that snapshot-based profiling is more meaningful than end-to-end profiles, since lock contention, I/O, etc. may happen during short, critical portions of execution.

\paragraph{Quartz: A Tool for Tuning Parallel Program Performance~\cite{DBLP:conf/sigmetrics/AndersonL90}}
Introduces ``normalized processor time'': time spent in code divided by the number of other processors that are concurrently busy. This approximates impact by attributing high cost to code that runs when a large fraction of other threads are blocked. This approximation will find bottlenecks on the critical path, and on sub-critical paths. Uses instrumentation.

\paragraph{Effective performance measurement and analysis of multithreaded applications~\cite{DBLP:conf/ppopp/TallentM09}}
This is a sampling call-graph profiler that attributes samples to one of three categories: work, where useful work is being done; idle, where a thread is blocked on some shared resource; and overhead, where operations for managing parallelism are being performed. The Cilk runtime is instrumented to properly attribute samples to the "overhead" category. The focus of this work is on improving scalability.

\paragraph{CPPROFJ: Aspect-Capable Call Path Profiling of Multi-Threaded Java Applications~\cite{DBLP:conf/kbse/Hall02}}
Lots of extra work to support aspects. The relevant work is the multi-threaded extension to call-path profiling. Time is broken down into several categories: running; sharing with equal priority threads; waiting for higher priority threads; waiting for a monitor; and idle time blocked on other events.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{Tracing}

\paragraph{Performance debugging for distributed systems of black boxes~\cite{DBLP:conf/sosp/AguileraMWRM03}}
Uses message-level traces to infer causal paths through the system. Works for either RPC-style traces (with call-response message pairs) or arbitrary messages. Can use network-level mechanisms to collect traces "for free." Validate inferred paths by tagging messages with causal paths to establish ground truth.

\paragraph{X-Trace: A Pervasive Network Tracing Framework~\cite{DBLP:conf/nsdi/FonsecaPKSS07}}
Instrumentation for tracing requests through a networked system. Requires interposition on all mechanisms for interaction.

% TO ADD
\paragraph{A Distributed Programs Monitor for Berkeley UNIX~\cite{DBLP:conf/icdcs/MillerMS85}}
Traces signals, I/O, and network communication in UNIX systems.

% TO ADD
\paragraph{Monit: A Performance Monitoring Tool for Parallel and Pseudo-Parallel Programs~\cite{DBLP:conf/sigmetrics/KerolaS87}}
Traces process creation and exit, process activity, and system variables (memory used, scheduler queue length, etc).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{Critical Path Profiling}

\paragraph{Critical Path Analysis for the Execution of Parallel and Distributed Programs~\cite{DBLP:conf/icdcs/YangM88}}
Explicitly constructs a critical path by tracing a message-passing API.

\paragraph{Parallel Program Performance Metrics: A Comparison and Validation~\cite{DBLP:conf/sc/HollingsworthM92}}
Introduces \emph{slack}: a new metric, which measures the difference in lengths between the critical path and 2nd-longest path. Slack will be zero for a completely balanced parallel application. If a procedure on the critical path is also on the longest sub-critical path, improving its performance will improve whole-program performance. Slack does not account for this effect.

Also introduces \emph{logical zeroing}: a manipulation of the program activity graph, where execution times for each use of a procedure are set to zero. This measures the true impact of fixing a procedure, but requires a program activity graph.

They evaluate the above performance metrics, along with UNIX-style profiling, critical path profiling, and Quartz-NPT profiling (time attribution) using ``true zeroing.'' True zeroing requires complete removal of a procedure from the execution. If the procedure has side effects, this can be quite difficult. This is not an automatic, general approach but the result is similar to Causal's ``speedup'' experiments. They conclude that critical path profiling is the best metric (correlated with true zeroing) but all are valuable. No consideration of interaction between a "zeroed" procedure and concurrent execution (false sharing, contention, etc.), and no discussion of how accurate the true zeroing approach is when a procedure may have side effects.

They make a similar argument about the problem with gprof-style profiling: it doesn't distinguish between time spent busy waiting versus doing useful work.

\paragraph{An online computation of critical path profiling~\cite{DBLP:conf/spdt/Hollingsworth96}}
Constructs a critical path online, and performs critical path zeroing to measure the impact of potential optimizations. Requires instrumentation for edges in the program activity graph.

\paragraph{Critical Path Profiling of Message Passing and Shared-Memory Programs~\cite{DBLP:journals/tpds/Hollingsworth98}}
Uses Paradyn to instrument shared memory programs. Critical path is constructed by tracing edges in the program activity graph. Only works for communication via synchronization operations, and only supports spinlocks and barriers. Results show a significant difference between UNIX-style profiling and critical path profiling results.

\paragraph{Using Interaction Costs for Microarchitectural Bottleneck Analysis~\cite{DBLP:conf/micro/FieldsBHN03}}
This approach constructs a graph of operations at a hardware level. A potential optimization is evaluated by constructing an ``idealized'' graph, where edges for the dependence being optimized are shortened. The new critical path length is computed to predict the speedup. This leads to the same result as our approach, but requires an accurate measurement of the entire dependence graph.

\paragraph{Online Critical Path Profiling for Parallel Applications~\cite{DBLP:conf/cluster/ZhuBM05}}
Online performance evaluation for MPI. Establishes causality with blocking versus non-blocking MPI calls. Only examines inter-node performance bottlenecks.

% TO ADD
\paragraph{Online Computation of Critical Paths for Multithreaded Languages~\cite{DBLP:conf/ipps/OyamaTY00}}
Online critical path computation for a language with first-class threads and synchronization.

% TO ADD
\paragraph{Space-efficient time-series call-path profiling of parallel applications~\cite{DBLP:conf/sc/SzebenyiWW09}}
More MPI profiling/tracing. Emphasis on compression.

% TO ADD
\paragraph{AppInsight: mobile app performance monitoring in the wild~\cite{ravindranath2012appinsight}}
Interposes on event handling routines on mobile apps to identify the critical path for each event transaction. Captures thread interaction through signaling, but not shared memory.

% TO ADD
\paragraph{Portable and architecture independent parallel performance~\cite{DBLP:conf/pdp/HillJSV98}}
Generalizes call-path profiling to bulk-synchronous-parallel programs. Identifies unbalanced parallelism and the critical path.

% TO ADD
\paragraph{IPS: An Interactive and Automatic Performance Measurement~\cite{DBLP:conf/icdcs/MillerY87}}
Discuss with IPS-2.

% TO ADD
\paragraph{IPS-2: The Second Generation of a Parallel Program Measurement~\cite{DBLP:journals/tpds/MillerCHKLT90}}
Profiling for distributed systems, with support for the entire stack: from instructions up to network interactions. Traces process interaction events using shared memory. Critical path (and sub-critical paths) are identified. Prospective points for optimization are identified with zeroing.

% TO ADD
\paragraph{Performance Measurement for Parallel and Distributed Programs: A Structured and Automatic Approach~\cite{DBLP:journals/tse/YangM89}}
More critical path analysis (IPS-flavor).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{Potential Parallelism}

\paragraph{Kremlin: rethinking and rebooting gprof for the multicore age~\cite{DBLP:conf/pldi/GarciaJLT11}}
Kremlin is a profiler for serial programs, but identifies good areas for parallelization. Static instrumentation is inserted to track dynamic data dependencies. This ``hierarchical critical path analysis'' enables a straightforward application of Amdahl's law to predict potential speedup from parallelizing a region.

% TO ADD
\paragraph{Alchemist: A Transparent Dependence Distance Profiling Infrastructure~\cite{DBLP:conf/cgo/ZhangNJ09}}
Profiler for memory reuse distance, aimed at identifying code with parallelization potential.

% TO ADD
\paragraph{Modeling optimistic concurrency using quantitative dependence~\cite{DBLP:conf/ppopp/PraunBC08}}
Measures the degree of data dependence for potential parallelism with transactional memory.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{Scalability}

\paragraph{Input-sensitive Profiling~\cite{DBLP:conf/pldi/CoppaDF12}}
Profiling with a Valgrind tool that accounts for input size in profiles.

\paragraph{Algorithmic profiling~\cite{DBLP:conf/pldi/ZaparanuksH12}}
Single-threaded profiler for estimating algorithmic complexity. Uses instrumentation to construct a representation of repeated sections in the algorthm (steps), and correlates this with input size.

\paragraph{The Cilkview scalability analyzer~\cite{DBLP:conf/spaa/HeLL10}}
Profiling for scalability.

% TO ADD
\paragraph{Differential Profiling~\cite{DBLP:conf/mascots/McKenney95}}
Collect profiles for parallel programs at different loads. Extrapolates to determine how time spent thrashing, in critical sections, etc varies as the load is scaled up.

% TO ADD
\paragraph{Bottleneck identification and scheduling in multithreaded applications~\cite{DBLP:conf/asplos/JoaoSMP12}}
Identifies serial bottlenecks with help from programmers. Scalability is improved by offloading computation to a faster core during important bottlenecks.

% TO ADD
\paragraph{Towards architecture independent metrics for multicore performance analysis~\cite{DBLP:journals/sigmetrics/KulkarniPS10}}
Generalizes reuse distance to multicore programs. Uses a sampling approach to compute reuse distance for a subset of accesses. Measures shared memory communication between threads with an execution trace. Focus is on general metrics rather than architecture-specific details.

% TO ADD
\paragraph{Cautious, machine-independent performance tuning for shared-memory multiprocessors~\cite{talbot1996cautious}}
Reports the potential for cache-level contention from program traces. Emphasis on scaling up input size.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{Bottleneck Identification}

% TO ADD
\paragraph{Thread Performance: Resource Contention Concurrency Profiling in Visual Studio 2010~\cite{goldin2010thread}}
Measures the amount of time threads spend blocked on critical sections, broken down by thread, lock, and critical section.

% TO ADD
\paragraph{Evaluation and optimization of multicore performance bottlenecks in supercomputing applications~\cite{DBLP:conf/ispass/DiamondBMKKB11}}
Profile analysis oriented toward scalability. Relies on L1/L2/L3 cache miss rates, IPC, and other hardware performance counter metrics.

% TO ADD
\paragraph{PerfExpert: An Easy-to-Use Performance Diagnosis Tool for HPC Applications~\cite{DBLP:conf/sc/BurtscherKDMKB10}}
Uses HPCToolkit to measure local performance metrics (like ``local cycles per-instruction'') at procedure or loop granularity. Analysis can identify general problem categories like ``data accesses'' and ``floating-point instructions'' and makes general suggestions. Specifically looks at hardware-level bottlenecks (including bus-level), and does not account for critical versus sub-critical paths.

% TO ADD
\paragraph{The Paradyn Parallel Performance Measurement Tool~\cite{DBLP:journals/computer/MillerCCHIKKN95}}
Evaluates a set of performance hypotheses automatically. Quite general: can handle distributed or local, locks/semaphores or messages, all for long-running applications. Requires a set of hypotheses, and mechanism must be adapted to handle each type of bottleneck. Paradyn makes no prediction about the impact of removing a bottleneck. The approach may identify bottlenecks that are off the critical path, but I'm not positive.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{Performance Experimentation}

% TO ADD
\paragraph{Evaluating the accuracy of Java profilers~\cite{DBLP:conf/pldi/MytkowiczDHS10}}
The authors find that existing Java profilers do not properly convey the importance of specific methods to program performance, in \emph{serial programs}. They find that existing profilers use garbage collection safe-points to collect profile samples, which biases the results. They establish this, validate output of their own unbiased profiler by inserting delays into the program and measuring the impact of removing the delay.

% TO ADD
\paragraph{Synthetic-perturbation Techniques for Screening Shared Memory Programs~\cite{DBLP:journals/spe/SnelickJKL94}}
Insert delays, run programs, measure performance impact. Captures marginal impact, but not peak impact. Requires many runs.

% TO ADD
\paragraph{An Active Approach to Characterizing Dynamic Dependencies for Problem Determination in a Distributed Environment~\cite{DBLP:conf/im/BrownKK01}}
Introduces a technique called ``Active Dependence Discovery.'' ADD relies on an enumeration of all components in a distributed system that may affect performance. ADD perturbs the performance at each component and measures the resulting effect on response time. Perturbations are inserted on a per-application basis (they perturb a database interface by changing the code to use a global lock rather than per-table or per-row locks). ADD discovers dependencies, but this work does not address root-cause analysis, nor does it make performance predictions.

% TO ADD
\paragraph{Finding and Removing Performance Bottlenecks in Large Systems~\cite{DBLP:conf/ecoop/AmmonsCGS04}}
Provide a mechanism for comparing call context trees from two different configurations of a program. When the tree is "more expensive" in one configuration, it can identify the component of the tree that is responsible. Strictly a post-processing framework.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{For Later}

\paragraph{Understanding and detecting real-world performance bugs~\cite{DBLP:conf/pldi/JinSSSL12}}

\paragraph{Catch me if you can: performance bug detection in the wild~\cite{DBLP:conf/oopsla/JovicAH11}}

\paragraph{Critical-path planning and scheduling: Mathematical basis~\cite{kelley1961critical}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{In Progress}



%\subsection*{Not Relevant}
%\begin{itemize}
%	\item Dependency Analysis in Distributed Systems using Fault Injection: Application to Problem Determination in an e-commerce Environment~\cite{DBLP:conf/dsom/BagchiKH01}
%	\item Shared memory programming for large scale machines~\cite{DBLP:conf/pldi/BartonCAZFCA06}
%	\item ParaProf: A Portable, Extensible, and Scalable Tool for Parallel Performance Profile Analysis~\cite{DBLP:conf/europar/BellMS03} \emph{Bold, but untested claims. This paper is about a UI, nothing else. References the TAU performance system, which doesn't seem to be described anywhere.}
%	\item Performance and environment monitoring for continuous program optimization~\cite{DBLP:journals/ibmrd/CascavalDSW06} \emph{Just another hardware performance counter visualization tool. Nothing new here.}
%	\item Kremlin: like gprof, but for parallelization~\cite{DBLP:conf/ppopp/JeonGLVT11} \emph{This is just an extended abstract}
% 	\item A Practical Method for Quickly Evaluating Program Optimizations~\cite{DBLP:conf/hipeac/FursinCOT05} \emph{I probably just clicked this because it's relevant to Stabilizer.}
%	\item Efficient online detection of dynamic control dependence~\cite{DBLP:conf/issta/XinZ07} \emph{Not relevant at all. Must have been a mistake.}
%	\item The Integration of Application and System Based Metrics in a Parallel Program Performance Tool~\cite{DBLP:conf/ppopp/HollingsworthIM91} \emph{Just an extension of IPS-2. Nothing parallel-specific here.}
%	\item Shadow Profiling: Hiding Instrumentation Costs with Parallelism~\cite{DBLP:conf/cgo/MoseleySRGP07} \emph{Nothing about profiling for parallelism. They just use parallelism to reduce instrumentation overhead.}
%	\item Reducing power with dynamic critical path information~\cite{DBLP:conf/micro/SengTT01} \emph{Interesting, but not really relevant. They use an online critical path computation to send critical instructions to higher-power functional units.}
%\end{itemize}
%	\item Analyzing software performance in a multiprocessor environment~\cite{maples1985analyzing} \emph{Measurement of scalability for the Othello game. Tuning work is all guided by developer insight.}
%	\item Causeway: Operating System Support for Controlling and Analyzing the Execution of Distributed Programs~\cite{DBLP:conf/hotos/ChandaECZ05} \emph{Proposes a tracing-based profiler for programs written using Causeway's distributed and parallel actor model. They don't actually implement it though.}



==> related_table.tex <==
\begin{table*}[t]
	\centering
	\small
	\begin{tabular}{ r | c c |  }
			& \multicolumn{2}{c|}{\bf{Mechanism}}	\\
			& \it{Instrumentation}	& \it{Sampling}	\\
		\hline
		\texttt{gprof}~\cite{DBLP:conf/sigplan/GrahamKM82}
			& \yes					& \yes			\\
		
		\texttt{oprofile}~\cite{oprofile}
			& \no					& \yes			\\
		
		Visual Studio Contention Profiler~\cite{goldin2010thread}
			& \yes					& \no			\\

		\hline
		\toolname{}
			& \yes					& \yes			\\
	
	\end{tabular}
	\caption{
		Prior work
		\label{tab:related}
	}
\end{table*}

==> writing_tasks.tex <==
\section{Writing Tasks}

% TODO Add Citations?
  
  % http://daniel-wilkerson.appspot.com/trend-prof.pdf
  
  % http://research.cs.wisc.edu/wind/Publications/centera-isca05.pdf
  
  % HPCToolkit - http://dl.acm.org/citation.cfm?id=1753233
  
  % Lamport on Causality - ?
  
  % Compiler-Driven Dependence Profiling to Guide Program Parallelization - http://link.springer.com/chapter/10.1007%2F978-3-540-89740-8_16
  
  % Performance and environment monitoring for continuous program optimization - http://ieeexplore.ieee.org/xpl/articleDetails.jsp?arnumber=5388726
  
  % Performance regression testing target prioritization via performance risk analysis - http://dl.acm.org/citation.cfm?doid=2568225.2568232
  
  % Continuous profiling: where have all the cycles gone? - http://dl.acm.org/citation.cfm?id=265925
  
  % A Dynamic Tracing Mechanism for Performance Analysis of OpenMP Applications - http://link.springer.com/chapter/10.1007%2F3-540-44587-0_6
  
  % Memphis: Finding and fixing NUMA-related performance problems on multi-core platforms - http://ieeexplore.ieee.org/xpl/articleDetails.jsp?arnumber=5452060
  
  % Exploiting statistical correlations for proactive prediction of program behaviors - http://dl.acm.org/citation.cfm?doid=1772954.1772989
  
  % Criticality stacks: identifying critical threads in parallel programs using synchronization behavior - http://dl.acm.org/citation.cfm?doid=2485922.2485966
  
  % Full-System Critical Path Analysis - http://ieeexplore.ieee.org/xpl/articleDetails.jsp?arnumber=4510739
  
  % End-to-end performance forecasting: finding bottlenecks before they happen - http://dl.acm.org/citation.cfm?doid=1555754.1555800
  
  % Cache Profiling and the SPEC Benchmarks: A Case Study - http://www.computer.org/csdl/mags/co/1994/10/rx015-abs.html
  
  % Performance debugging shared memory parallel programs using run-time dependence analysis - http://dl.acm.org/citation.cfm?doid=258612.258678 

